See and Think: Embodied Agent in Virtual Environment

Large language models (LLMs) have achieved impressive pro-gress on several open-world tasks. Recently, using LLMs to build embodied agents has been a hotspot. This paper proposes STEVE, a comprehensive and visionary embodied agent in the Minecraft virtual environment. STEVE comprises three key components: vision perception, language instruction, and code action. Vision perception involves interpreting visual information in the environment, which is then integrated into the LLMs component with agent state and task instruction. Language instruction is responsible for iterative reasoning and decomposing complex tasks into manageable guidelines. Code action generates executable skill actions based on retrieval in skill database, enabling the agent to interact effectively within the Minecraft environment. We also collect STEVE-21K dataset, which includes 600+ vision-environment pairs, 20K knowledge question-answering pairs, and 200+ skill-code pairs. We conduct continuous block search, knowledge question and answering, and tech tree mastery to evaluate the performance. Extensive experiments show that STEVE achieves at most 1.5x faster unlocking key tech trees and 2.5x quicker in block search tasks.

==> prompt/Decompose.tex <==
\begin{tcolorbox}[breakable=true, boxrule={0.5pt}, sharp corners={all}]
\setlength{\parskip}{1ex}
\textbf{SYSTEM:}

You are designated as an assistant for the game Minecraft. Your task involves formulating goals related to obtaining specific objects within the game. I'll provide you with a specific target and relevant extensive information. Please provide a standardized format for acquiring this target as a goal.

Goal Structure: \\
\{\\
  ``object'': ``[Name of Target Object]'',\\
  ``amount'': [Target Amount],\\
  ``material'': \{ \\
  \hbox{\ \ \ \ \ \ \ \ }[Material Name]: [Material Quantity], \\
  \hbox{\ \ \ \ \ \ \ \ } ... \\
  \hbox{\ \ \ \ }\},\\
  ``tool'': ``[Tool Required]'',\\
  ``info'': ``[Concise Information Related to the Goal]''\\
\}\\
\hbox{\ \ \ \ }- Target: Enter the name of the target object you wish to obtain or craft.,\\
\hbox{\ \ \ \ }- Amount: Specify the amount of the target object needed.,\\
\hbox{\ \ \ \ }- Material: List the materials required to achieve this goal. Format each entry as "material name": quantity. If no material is required, set this field to None,\\
\hbox{\ \ \ \ }- Tool: Indicate the most basic tool necessary for this goal. If multiple tools can be used, choose the simplest one. If no tool is required, set this to None,\\
\hbox{\ \ \ \ }- Info: Provide essential information related to the goal. Summarize the knowledge in up to three sentences, focusing on key details about obtaining or crafting the target object.\\

Requirements:\\
1. Goals must be constructed based on the provided knowledge, rather than relying solely on pre-existing knowledge.\\
2. The "info" section should be concise and informative, limited to a maximum of three sentences. Extracting and summarizing the key information from the provided knowledge is essential, rather than replicating the entire text.\\

Example Goal 1:\\
\{\\
\hbox{\ \ \ \ }``target'': ``bed'',\\
\hbox{\ \ \ \ }``amount'': 1,\\
\hbox{\ \ \ \ }``material'': \{``wool'': 3, ``planks'': 3\},\\
\hbox{\ \ \ \ }``tool'': ``crafting table'',\\
\hbox{\ \ \ \ }``info'': ``A bed is crafted using 3 wool and 3 wooden planks on a crafting table. Beds allow players to skip the night and reset their spawn point.''\\
\}\\
Example Goal 2:\\
\{\\
\hbox{\ \ \ \ }``target'': ``paper'',\\
\hbox{\ \ \ \ }``amount'': 3,\\
\hbox{\ \ \ \ }``material'': \{"sugar cane": 3\},\\
\hbox{\ \ \ \ }``tool'': ``None'',\\
\hbox{\ \ \ \ }``info'': ``Paper is crafted from 3 sugar cane, arranged in a row. It's used for creating maps and books.''\\
\}\newline
\newline
\textbf{USER:}

Target info: \texttt{\{target amount\}} \texttt{\{target name\}}\\
Knowledge info: \texttt{\{extensive knowledge\}}
\end{tcolorbox}
% \twocolumn

==> prompt/generate_qa.tex <==
\begin{tcolorbox}[breakable=false, boxrule={0.5pt}, sharp corners={all}]
\setlength{\parskip}{1ex}
\textbf{SYSTEM:}

You are a helpful assistant engaging in a conversation with an in-game Minecraft agent. This agent seeks to enhance both its survival techniques and interaction tactics within the Minecraft universe.

Your task is to extract crucial questions and their corresponding answers from the provided Minecraft information. These may pertain to survival challenges, crafting recipes, interactions with in-game entities, and other relevant aspects.

\#\#INSTRUCTIONS:

- Craft questions to prompt the in-game Minecraft agent to contemplate various aspects of gameplay, including survival challenges, crafting recipes, managing resources, navigating terrain, interactions with in-game entities, and more. \\
- For each question, extract a suitable answer. Each answer should elucidate the agent's perspective, emphasizing effective strategies, item applications, or interaction approaches.

\textbf{USER:}
    
The information about Minecraft is: \texttt{\{text\}}.

Present your output in the mold of a Python dictionary string, utilizing `Q' for questions and `A' for the agent's anticipated responses. For multiple questions derived, maintain the 'Q' and 'A' structure. 

An example could be: `Q': `How to craft a wooden pickaxe in Minecraft?', `A': `To craft a wooden pickaxe, the approach involves...', `Q': `...', `A':`...', ... 

\end{tcolorbox}

==> prompt/score.tex <==
\begin{tcolorbox}[breakable=false, boxrule={0.5pt}, sharp corners={all}]
\setlength{\parskip}{1ex}
\textbf{SYSTEM:}

You are an intelligent chatbot designed for evaluating the correctness of generative outputs for question-answer pairs. 

Your task is to compare the predicted answer with the correct answer and determine if they match meaningfully. Here's how you can accomplish the task:

\#\#INSTRUCTIONS:

- Focus on the meaningful match between the predicted answer and the correct answer.\\
- Consider synonyms or paraphrases as valid matches.\\
- Evaluate the correctness of the prediction compared to the answer.

\textbf{USER:}

Please evaluate the following question-answer pair:\\
Question: \texttt{\{question\}}\\
Correct Answer: \texttt{\{ground truth\}} \\
Predicted Answer: \texttt{\{answer\}} 

Provide your evaluation only in the form of a score, where the score is an integer value between 0 and 10, with 10 indicating the highest meaningful match.

Do not provide any other output text or explanations. Only provide output score.
For example, your response should look like this: `9'.

\end{tcolorbox}



==> skills/skill-code.tex <==
% A full list of skills is included in the supplementary folder.
\renewcommand\lstlistingname{Skill-Code example}
\setcounter{lstlisting}{0}
\lstinputlisting[language=JavaScript,breaklines=true,caption=craftShieldImproved.]{skills/craftShieldImproved.js}
\clearpage
\lstinputlisting[language=JavaScript,breaklines=true,caption=craftBed.]{skills/craftBed.js}
\clearpage
\lstinputlisting[language=JavaScript,breaklines=true,caption=craftPaper.]{skills/craftPaper.js}
\lstinputlisting[language=JavaScript,breaklines=true,caption=craftShieldWithIron.]{skills/craftShieldWithIron.js}
\lstinputlisting[language=JavaScript,breaklines=true,caption=mineFiveLapisOres.]{skills/mineFiveLapisOres.js}
\lstinputlisting[language=JavaScript,breaklines=true,caption=smeltTwelveRawCopper.]{skills/smeltTwelveRawCopper.js}
\lstinputlisting[language=JavaScript,breaklines=true,caption=obtainTenWoodLogs.]{skills/obtainTenWoodLogs.js}

==> tab/LLM_efficiency.tex <==
\begin{table}[t!]
\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}[c]{l|c}
\toprule
Method & time(s)~($\downarrow$) \\ 
\midrule
Llama2-7B~\cite{gao2023llama} & 18.34\\
Llama2-13B~\cite{gao2023llama} & 21.17\\
GPT-4~\cite{openai2023gpt4} & 22.86\\
\textbf{STEVE-7B} & \textbf{7.19}\\
\bottomrule
\end{tabular}
}
\caption{
Comparison on \textbf{language model efficiency}. It shows the average time for each question-answering.}
\label{table:LLM_eff}
\end{table}

==> tab/comp_component.tex <==
\begin{table*}[!ht]
\vskip 0.1in
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{p{2cm}|p{1.5cm}|p{2.5cm}|p{2.5cm}|p{1.5cm}|p{2cm}|p{2cm}|p{2cm}}
    \toprule
    & VPT~\cite{openai2022vpt}& DreamerV3~\cite{hafner2023mastering} & DECKARD~\cite{nottingham2023embodied} & DEPS~\cite{wang2023describe} & Plan4MC~\cite{yuan2023plan4mc} & Voyager~\cite{wang2023voyager} &
    STEVE~(ours)\\
    \midrule
    Demos & Videos & None & Videos & None & None & None & Videos \\
    \midrule
    Rewards & Sparse & Dense & Sparse & None & Dense & None & None \\
    \midrule
    Observations & Pixels Only & \parbox[t]{2cm}{Pixels \& \\Meta} & \parbox[t]{2cm}{Pixels \& \\Inventory} & \parbox[t]{2cm}{Feedback \& \\Inventory} & \parbox[t]{2cm}{Pixels \& \\Meta} & \parbox[t]{2cm}{Feedback \& \\Meta \& \\Inventory} & \parbox[t]{2cm}{Pixels \& \\ Feedback \& \\Meta \& \\Inventory} \\
    \midrule
    Actions & Keyboard \& Mouse & Discrete & Keyboard \& Mouse & Keyboard \& Mouse & Discrete & Code & Code\\
    \midrule
    Iterative Planning & & & & $\checkmark$ & &$\checkmark$ & $\checkmark$ \\
    \midrule
    Skill Database & & & & & \parbox[t]{2cm}{9} & \parbox[t]{2cm}{172} & \parbox[t]{2cm}{210} \\
    \midrule
    Gradient-Free & & & & & & $\checkmark$ & $\checkmark$\\
    \bottomrule
    \end{tabular}
}
\caption{Comparison between \textbf{STEVE and representative works.} It is a system-level comparison consisting of LLM-based and RL-based methods.}
\label{table:comparison_component}
\end{table*}

==> tab/comp_rebuttal.tex <==
\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
     Method & LLM. & Perception & Training & Dataset \\
    % & steve-eye~\cite{zheng2023steve} & JARVIS-1~\cite{wang2023jarvis} & GROOT~\cite{cai2023groot}	& MC-controller~\cite{cai2023open}	& STEVE-1~\cite{lifshitz2023steve} & STEVE~(ours)\\
    \midrule
    Voyager & GPT-4-0613  & Meta, r $=$ 32 &- &-\\
    \midrule
    \textbf{STEVE~(ours)} & STEVE-13b &Ego RGB, r $=$ 256 & Online &simulation\\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Component comparison with Voyager.} Meta is the metadata from the background, Ego RGB is for Ego-view image, and r represents the maximal distance of perceived entities.}
\label{table:comparison_rebuttal}
\end{table}

==> tab/dataset.tex <==
\begin{table}[t]
\centering
% \scriptsize
\resizebox{1\linewidth}{!}{
\begin{tabular}[c]{l|cc|l}\toprule
Section & \# pairs & \# types &  \\ \midrule
Vision-Environment & 600 & 6 & video, environment, chat flow\\
Question-Answering & 20K & 6 & question, answer\\
Skill-Code & 210 & 8 & skill description, code, vectordb\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Statistics} of STEVE-20K, including the number of pairs, number of categories, and content.}
\label{table:dataset}
\end{table}



==> tab/exp_inst_single.tex <==
\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[c]{l|cccccc|c}
\toprule
Method  & World \& Entities & Player Mechanics \& Survival & Knowledge \& Discovery & Resources \& Crafting & Tools \& Utilities & Miscellaneous & Overall\\ 
\midrule
GPT-4 & 8.53 & 8.56 & \textbf{8.85} & 8.49 & 8.63 & \textbf{9.00} & 8.59\\
\midrule
Llama2-7B  & 7.22 & 7.43 & 7.12 & 7.01 & 7.28 & 8.45 & 7.23\\
Llama2-13B & 7.34 & 7.32 & 7.42	& 7.37 & 7.44 & 6.75 & 7.36\\
\midrule
\textbf{STEVE-7B} & 8.67 & 8.41 & 8.42 & 8.53 & 8.35 & 8.50 & 8.52\\
\textbf{STEVE-13B} & \textbf{8.74} & \textbf{8.67} & 8.72 & \textbf{8.68} & \textbf{8.74} & 7.95 & \textbf{8.70}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitive comparison on knowledge question and answering task by GPT-4~\cite{openai2023gpt4}.} It is rated on a scale of 0 to 10; Higher scores indicate greater alignment of the generated answers with the ground truth.}
\label{table:exp_inst_gpt}
\end{table*}


\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[c]{l|cccccc|c}
\toprule
Method  & World \& Entities & Player Mechanics \& Survival & Knowledge \& Discovery & Resources \& Crafting & Tools \& Utilities & Miscellaneous & Overall\\ 
\midrule
GPT-4 & 8.17 & 8.31 & \textbf{8.27} & 8.17 & \textbf{8.24} & 8.10 & 8.21\\
\midrule
Llama2-7B  & 6.76 & 6.94 & 6.90 & 6.60 & 7.10 & 6.85 & 6.83\\
Llama2-13B & 7.21 & 7.19 & 7.01 & 7.00 & 7.32 & 7.15 & 7.16\\
\midrule
\textbf{STEVE-7B} & 8.14 & 8.12 & 8.09 & 8.11 & 8.18 & 8.00 & 8.13\\
\textbf{STEVE-13B} & \textbf{8.24} & \textbf{8.34} & 8.21 & \textbf{8.24} & 8.20 & \textbf{8.15} & \textbf{8.24}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitive comparison on knowledge question and answering task by Claude-2~\cite{claude}.} It is rated on a scale of 0 to 10; Higher scores indicate greater alignment of the generated answers with the ground truth.}
\label{table:exp_inst_claude}
\end{table*}

\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[c]{l|cccccc|c}
\toprule
Method  & World \& Entities & Player Mechanics \& Survival & Knowledge \& Discovery & Resources \& Crafting & Tools \& Utilities & Miscellaneous & Overall\\ 
\midrule
GPT-4 & \textbf{7.48} & 7.33 & 7.08 & 7.11 & 7.39 & \textbf{7.52} & 7.32\\
\midrule
Llama2-7B  & 5.34 & 5.67 & 5.72 & 5.65 & 6.01 & 5.57 & 5.62\\
Llama2-13B & 6.23 & 6.35 & 5.89 & 5.94 & 6.19 & 6.02 & 6.14\\
\midrule
\textbf{STEVE-7B} & 7.15 & 7.11 & 7.01 & 7.22 & 7.27 & 6.97 & 7.16\\
\textbf{STEVE-13B} & 7.43 & \textbf{7.39} & \textbf{7.17} & \textbf{7.52} & \textbf{7.43} & 7.06 & \textbf{7.41}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitive comparison on knowledge question and answering task by human blind rating.} It is rated on a scale of 0 to 10; Higher scores indicate greater alignment of the generated answers with the ground truth.}
\label{table:exp_inst_human}
\end{table*}

==> tab/exp_pearson.tex <==
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[c]{l|c}
\toprule
Method & Pearson Correlation Coefficients \\ 
\midrule
GPT-4 VS. Claude-2 & 0.976\\
GPT-4 VS. Human Blind Rating & 0.965\\
Claude-2 VS. Human Blind Rating & 0.998\\
\bottomrule
\end{tabular}
}
\caption{
Comparison on \textbf{Pearson correlation coefficients between score methods}. It calculates the mean score across each score dimensions for each language methods and then computes the Pearson correlation between these means for each pair of score methods~(GPT-4, Claude-2 and Human blind rating). The Pearson correlation coefficient ranges from -1 to +1. Higher Pearson correlation coefficient (closer to +1) means that there is a stronger positive linear relationship between the two sets of data.}
\label{table:pearson}
\end{table}

==> tex/7_sup.tex <==
\appendix
\renewcommand\thefigure{\Alph{section}\arabic{figure}}
\renewcommand\thetable{\Alph{section}\arabic{table}}
\setcounter{figure}{0}
\setcounter{table}{0}

\paragraph{The supplementary material is structured as follows:}
\begin{itemize}
\item [$\bullet$] We begin with the ``Contribution and Idea'' of the STEVE to explain the reason of data collection and fine-tuning in~\cref{sec:contribution}.
\item [$\bullet$] Then, we introduce the ``STEVE Pseudo Code'' section, detailing the STEVE method, encompassing input requirements, variables, functions, and the procedure of the STEVE Method algorithm in~\cref{sec:pseudo}
\item [$\bullet$] Next, the ``Component Comparison'' section offers a comparison of the STEVE system with representative and concurrent works, focusing on various system characteristics such as availability of demos, nature of rewards, and types of observations, and even the specific core method differences and whether there is control capability, among others, in~\cref{sec:component}
\item [$\bullet$] The ``Implementation Detail'' section outlines the steps involved in implementing STEVE, including the warm-up with the Question-Answering pair, collection of Vision-Environment pair, and training and fine-tuning processes in~\cref{sec:implementation}.
\item [$\bullet$] In the ``STEVE-7B/13B'' section, we introduce the features and capabilities of the STEVE-7B/13B model, along with the Pearson correlation coefficient analysis for various score methods and showcases the efficiency of language models in the Minecraft knowledge QA domain, as shown in~\cref{sec:STEVE-7B/13B}.
\item [$\bullet$] The ``Prompt'' section provides insights into the LLM Decomposer, the process for generating Question-Answering pairs, and the evaluation methodology in~\cref{sec:prompt}.
\item [$\bullet$] The ``Demo Image and Video'' section presents practical demonstrations of STEVE in various tasks, supported by figures and video content, and examples of skills and code in~\cref{sec:demo}.
\item [$\bullet$] Lastly, the ``Skill-Code Example'' section contains examples from the STEVE-21K skill-code part, illustrating specific skill codes used in the STEVE system, as showvn in~\cref{sec:example}
\end{itemize}

\section{Contribution and Motivation}~\label{sec:contribution}
STEVE is the first \textbf{pure LLM-based} embodied agent with \textbf{vision perception} and \textbf{comprehensive control capabilities}, as shown in Table~\ref{table:comparison_rebuttal}. We get \textbf{SOTA} performance as an LLM-based model, providing excellent performance in visual perception and \textbf{interpretable planning} (Section 5.3) with \textbf{flexibility} on tasks. 
We explain why we collect data and fine-tune a smaller LLM instead of relying solely on GPT-4 as follows.

\noindent\textbf{(1) Innovative embodied agent tasks with a smaller LLM:} We showed that complex tasks can be done with few LLM parameters while ensuring interpretability. This is necessary for cost-effective solutions. STEVE-7B/13B has better efficiency than GPT-4, achieving SOTA performance by adding visual perception. Our work verifies that models with small parameter quantities can perform well beyond models with extremely large parameter quantities through simple finetuning on a specific domain. Although it may sacrifice some performance in unseen scenarios, it is common for most non-gradient-free and finetuned LLM methods, as shown in Table~\ref{table:comparison_rebuttal}.

\noindent\textbf{(2) Superior performance and vision integration:} Our work enhances the SOTA LLM-based model Voyager with visual capabilities. STEVE has shown a significant performance boost in tasks like tech tree mastery and block searching, suggesting potential improvements in navigation tasks. This approach bridges the gap between virtual environments and the real world for embodied agents. We train the vision encoder with object-level labels, providing fine-grained recognition.

\noindent\textbf{(3) Multi-role collaboration in language instruction:} The Language Instruction system, composed of different roles of the STEVE-7B/13B model (Planner, Critic, Curriculum, and Describer) with buffer to manage tasks in Minecraft by formulating long-term plans, refining strategies through feedback, adapting via a curriculum of complex tasks, and translating strategies into executable textual actions.

\noindent\textbf{(4) Online training via simulation:} We provide online training for visual encoders, multi-role language models, and agent simulation for faster and more realistic training. No need for separate visual and language model training or offline strategies.

\noindent\textbf{(5) Cost-effectiveness lightweight and sustainable development:} Many methods rely directly on GPT-4, combined with RL model. The fine-tuning process LoRA we employed is cost-effective without any API expense. STEVE is also very lightweight because using only the 7B/13B model without other additional models will not bring additional costs, and it also has control capabilities. STEVE will be open-source, reducing ongoing development expenses. This makes our model more practical for complex tasks such as RLEF~(Environment Feedback) and Role Agents.

\noindent\textbf{(6) Value of the dataset:} We contribute a comprehensive multimodal dataset of \textbf{actual simulation} that spans visual perception, knowledge instruction, and action execution. This dataset has 20K Minecraft question-answering text pairs, 600 vision-environment pairs including more than \textbf{\textit{36K}} temporal frames with corresponding environment information and LLM context,  and 210 skill code snippets with descriptions~(GPT generation). We collect a comprehensive dataset including simulation (vision-environment-chatflow), instruction (Knowledge QA), and skill codebase. 

\section{STEVE Pseudo Code}~\label{sec:pseudo}
STEVE takes an image, the agent's current state, and a task as inputs, and uses a series of functions like a vision encoder, text tokenizer, and the core STEVE-7B/13B model to process these inputs. The model generates a plan consisting of steps, each of which is decomposed into an executable format, encoded into a query, and then used to retrieve an action code from a skill database. This process ultimately produces a series of action codes that guide the agent in performing the specified task.

\begin{algorithm}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \caption{STEVE Method~$F$}
    \label{alg:STEVE}
    \begin{algorithmic}[1]
    \Require Image $\mathcal{I}$, Agent State $\mathcal{S}$, Task $\mathcal{T}$
    \State \textbf{Variables:}
        \State \quad $step_e$: Executable step
        \State \quad $q$: Action query
        \State \quad $a$: Action code
    \State \textbf{Functions:}
        \State \quad $V$: Vision encoder
        \State \quad $T$: Tokenizer for text
        \State \quad $S$: STEVE-7B/13B
        \State \quad $E$: Query encoder
        \State \quad $R$: Retrieval module on Skill Database
    \Procedure{$F$}{$\mathcal{I}$, $\mathcal{S}$, $\mathcal{T}$}
        \State $O_V \gets V(\mathcal{I})$
        \State $O_S \gets T(\mathcal{S})$
        \State $O_T \gets T(\mathcal{T})$
        \State $P_H \gets S(O_V, O_S, O_T)$
        \For{each $step$ in $P_H$}
            \State $step_e \gets Decompose(step)$
            \State $Query \gets E(step_e)$
            \State $a \gets R(Query)$
        \EndFor
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

\section{Component Comparison}~\label{sec:component}
\input{tab/comp_component}
\input{tab/comp_rebuttal}
As shown in~\cref{table:comparison_component}, we compare STEVE with several existing works in the field. We consider the following characteristics of each system: availability of demos, nature of rewards, types of observations, action form, use of iterative planning, existence and capacity of a skill database, and whether they are gradient-free. 
As shown in~\Cref{table:comparison_rebuttal}, our STEVE uses Ego-view RGB to directly perceive visual information within a 256-block range, enhancing realism and directional sensitivity. It also features \textbf{unique multi-role} language models with continuous learning for long-term planning and task adaptation.

We also compare agents using non-pure LLM and RL, excelling in environments with defined objectives but challenging to address open-ended tasks. Our STEVE is designed for open-ended tasks with varying language-based objectives, operating autonomously in the unrestricted Minecraft environment, contrasting with RL agents confined to specific settings like Minedojo. As a loose comparison, it achieves a 19\% success rate in the Diamond Tool task within 10 minutes, surpassing RL-based VPT~\cite{baker2022video} at 12\%.

\section{Implementation Detail}~\label{sec:implementation}

\noindent\textbf{(1) RayTracing module:} Raytracing is a perception module we developed. Through this module, we can ensure that all content outside the robot's perspective screen is eliminated and only all visible blocks and entities are saved. Note that it is only used to collect data. This module is removed in STEVE since a vision encoder is used for perception.


\noindent\textbf{(2) LLM warm-up:} We use LoRA finetuning on the 20K Knowledge QA pairs of STEVE-21K, using LLaMA2-7B/13B, before being deployed in a simulated environment. The warm-up step is a one-time process that allows the model to absorb extensive knowledge. It is a crucial step in the initial simulation, which enables the collection of the vision-environment pair.

\noindent\textbf{(3) Second stage of LLM finetuning:} We simulate STEVE-13B in Minecraft, a simple embodied agent that uses the RayTracing module directly. After 5,000 simulations, we collected context information from successful runs, including sequences of QA. We then use these to fine-tune STEVE-13B via the LoRA process. Note that the process is to adjust STEVE-13B to work on \textbf{correct simulation knowledge} while remaining \textbf{adapted to visual perception}.

\noindent\textbf{(4) Vision-environment pair collection:} We run STEVE-13B with a second-round Minecraft simulation. We recorded 600 \textbf{videos}, collected environmental data with RayTracing, saved state information, and chatflow. We collect the dataset in six different terrains: forest, desert, coastal, \etc. We use the STEVE-7B/13B model to enable robots to autonomously plan and execute actions based on tasks defined by human supervisors. We record the video of the robot operation, environment information, and all the corresponding chat flow. Note that we use ray tracing~\cite{whitted2005improved} to ensure the environmental information obtained is the blocks and entities seen in the field of vision.

\noindent\textbf{(5) Multi-role instruction:} The Planner uses visual information for task decomposition and sequencing, while the Critic, inspired by Voyager, provides essential error correction. The Curriculum stores extensive semantic information to support continuous learning and preserve effective task sequences. Lastly, the Describer, influenced by the chain of summarization~\cite{ma2023large}, condenses historical data to improve long-term memory.

\noindent\textbf{(6) STEVE-21K dataset:} It is not only specifically tailored for training our STEVE system but is used as the foundation for developing STEVE from scratch, utilizing the open-source LLaMA as the base model. The dataset contains visual environment data and contextual LLM QA pairs, with 50\% used for real-time learning and the rest for diversity. STEVE-21K effectively trains STEVE, showing its potential for wider language model training.

\noindent\textbf{(7) Experiment and evaluation:} We propose Continuous Block Search, Knowledge QA, and Tech Tree Mastery (Section 5.3). Our model has achieved SOTA results in each domain. 
\textbf{Continuous Block Search} enhances exploration abilities by evaluating the visual perception capabilities of the model. It is inspired by Voyager's map exploration tasks, emphasizing purpose-driven searches influenced by multimodal navigation tasks~\cite{wang2022towards}.
\textbf{Knowledge QA} explicitly demonstrates the language model's performance ~(more Language model efficiency details in Supplementary Material D.). LLM-based methods can reflect simulation performance to an extent. High QA performance can indicate high simulation performance and vice versa.
\textbf{Tech Tree Mastery} demonstrates the control capabilities. We use the same settings as the comparison method, including the code database.

\section{STEVE-7B/13B}~\label{sec:STEVE-7B/13B}
We propose STEVE-7B/13B, a powerful language model series derived from LLaMA2~\cite{gao2023llama}, fine-tuned specifically on Minecraft-related content from the Minecraft-wiki and Reddit corpus. This model's expertise covers a broad spectrum of game-specific knowledge areas including:

\begin{itemize}
    \item [$\bullet$] \textbf{World Understanding:} Geography, biomes, and entity interactions.
    \item [$\bullet$] \textbf{Player Mechanics:} Health management, combat, and mobility.
    \item [$\bullet$] \textbf{Survival Strategies:} Food sourcing, shelter building, and enemy evasion.
    \item [$\bullet$] \textbf{Resource Management:} Item gathering, mining techniques, and inventory optimization.
    \item [$\bullet$] \textbf{Crafting and Construction:} Recipe knowledge, item crafting, and structure creation.
    \item [$\bullet$] \textbf{Utility and Tool Usage:} Tool selection, item upgrades, and special abilities.
\end{itemize}

We test the performance of our STEVE-7B/13B on the above-mentioned functional indicators. The entire knowledge question and answering section of our paper used 1000 pairs that were divided from our STEVE-21K. Among these 1000 pairs, the categories World \& Entities, Player Mechanics \& Survival, Knowledge \& Discovery, Resources \& Crafting, Tools \& Utilities, and Miscellaneous are respectively 332, 152, 108, 219, 169, 20.

\subsection{Detailed evaluation}
\begin{figure*}[htbp]
\centering
\subfloat[\textbf{GPT-4 and Claude-2: 0.976}]{
      \label{fig:subfig1}\includegraphics[width=0.33\textwidth]{fig/claude2_gpt4.pdf}
}
\subfloat[\textbf{GPT-4 and Human Blind Rating: 0.965}]{
      \label{fig:subfig1}\includegraphics[width=0.33\textwidth]{fig/GPT4_HumanBlindRating.pdf}
}
\subfloat[\textbf{Claude-2 and Human Blind Rating: 0.998}]{
      \label{fig:subfig1}\includegraphics[width=0.33\textwidth]{fig/Claude2_HumanBlindRating.pdf}
}
\centering
\caption{Pearson Correlation Analysis, including scatters and trend. Note that all scatters come from~\cref{table:exp_inst_gpt}~\ref{table:exp_inst_claude}~\ref{table:exp_inst_human}}
\end{figure*}
\input{tab/exp_inst_single}



\paragraph{Pearson correlation coefficient on score methods.} 
The formula represents the Pearson correlation coefficient:

\[
r_{xy} = \frac{\sum_{i=1}^{n}(x_i - \bar{x})(y_i - \bar{y})}{\sqrt{\sum_{i=1}^{n}(x_i - \bar{x})^2}\sqrt{\sum_{i=1}^{n}(y_i - \bar{y})^2}}
\]

where:

\begin{itemize}
    \item [$\bullet$] \( r_{xy} \) is the Pearson correlation coefficient between two variables \( x \) and \( y \).
    \item [$\bullet$] \( x_i \) and \( y_i \) are the individual sample points for variables \( x \) and \( y \), respectively.
    \item [$\bullet$] \( \bar{x} \) and \( \bar{y} \) are the means (averages) of the \( x \) and \( y \) samples, respectively.
    \item [$\bullet$] \( n \) is the number of sample points.
\end{itemize}

This formula essentially measures the degree of linear relationship between two variables. It compares the product of their deviations from their respective means. The numerator captures the covariance between the two variables, and the denominator normalizes this value, ensuring that the coefficient remains between -1 and +1. The Pearson correlation coefficient measures how much two variables change together compared to how much they vary individually.

As shown in~\cref{table:pearson}, the Pearson correlation coefficients are calculated between these methods: GPT-4 vs. Claude-2 (0.976), GPT-4 vs. Human Blind Rating (0.965), and Claude-2 vs. Human Blind Rating (0.998). It suggests a high level of agreement among these evaluation approaches. The alignment of scores from different evaluation methods reinforces the reliability of our assessment. Our STEVE models outperform other language models in knowledge question and answering tasks, including the benchmark GPT-4. This superior performance of STEVE, particularly the 13B version, is evident across a broad spectrum of categories. This suggests that our model has a deeper understanding of Minecraft-related content and exhibits a more accurate and consistent ability to generate relevant responses. 
\input{tab/exp_pearson}

\subsection{Language model efficiency}
We primarily test the reasoning efficiency of large language models on Minecraft knowledge QA and showcased case studies.
\input{tab/LLM_efficiency}
We conduct this experiment in the Question-Answering part of our STEVE-21K dataset.
As shown in~\cref{table:LLM_eff}, our model STEVE-7B/13B achieves leading performance in terms of time cost. This is due to its smaller number of parameters compared to GPT-4, and its shorter yet more accurate responses compared to the Llama series.

\section{Prompt}~\label{sec:prompt}

\subsection{LLM Decomposer}

We use STEVE-7B/13B for goal decomposition.
The format of the prompt is presented thus: directions under the "SYSTEM" role and questions under the "USER" role.
The \texttt{\{target amount\}}, \texttt{\{target name\}} and \texttt{\{extensive knowledge\}} are designed to be filled with specific content, which will then be inputted into the language model after substitution.

\subsection{Generate Question-Answering pairs}
We employ the following prompt during the collection of Question-Answer pairs. In this context, the placeholder \texttt{\{text\}} is intended to be filled with cleaned Minecraft-Wiki text.

\subsection{Evaluation}
We utilize GPT-4 and Claude-2 to evaluate various models, employing the following prompt structure. Within this structure, the placeholders \texttt{\{question\}}, \texttt{\{ground truth\}}, and \texttt{\{answer\}} are designated to be filled with questions, standard answers, and model-generated answers, respectively.

\section{Demo Image and Video}~\label{sec:demo}
As shown in~\cref{fig:basic_skill}, we experiment with our STEVE on various practical tasks, covering collecting, combating, mining~\etc. 

\section{Examples}~\label{sec:example}
The section contains examples from the STEVE-21K skill-code part, illustrating specific skill codes used in the STEVE system.

\input{prompt/Decompose}
\input{prompt/generate_qa}
\input{prompt/score}
\input{skills/skill-code}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/basic_skill.pdf}
    \caption{\textbf{Demo of basic survival skills.} }
    \label{fig:basic_skill}
\end{figure}
% \label{supp:sec:curriculum_prompt}
% \lstinputlisting[breaklines=true,caption={Full system prompt for automatic curriculum. The list of question-answer pairs represents the additional context.}]{appendix/prompts/curriculum_prompt.txt}
% \label{supp:sec:curriculum_prompt-curriculum}
